PPM: Automated Generation of Diverse Programming Problems for Benchmarking Code Generation Models

In recent times, a plethora of Large Code Generation Models (LCGMs) have been proposed, showcasing significant potential in assisting developers with complex programming tasks. Benchmarking LCGMs necessitates the creation of a set of diverse programming problems, and each problem comprises the prompt (including the task description), canonical solution, and test inputs. The existing methods for constructing such a problem set can be categorized into two main types: manual methods and perturbation-based methods. However, manual methods demand high effort and lack scalability, while also risking data integrity due to LCGMs' potentially contaminated data collection, and perturbation-based approaches mainly generate semantically homogeneous problems with the same canonical solutions and introduce typos that can be easily auto-corrected by IDE, making them ineffective and unrealistic. In this work, we propose the idea of programming problem merging (PPM) and provide two implementation of this idea, we utilize our tool on two widely-used datasets and compare it against nine baseline methods using eight code generation models. The results demonstrate the effectiveness of our tool in generating more challenging, diverse, and natural programming problems, comparing to the baselines.

==> Preliminary/results.tex <==
\subsection{Study Results}

==> Preliminary/setup.tex <==
\subsection{Study Setup}


==> Preliminary/study.tex <==
\subsection{Study Question}

==> Table/model.tex <==
% Table generated by Excel2LaTeX from sheet 'model info'
\begin{table*}[htbp]
  \centering
  \caption{The model architecture and the training information of code models}
  \vspace{-3mm}
  \resizebox{0.99\textwidth}{!}{
    \begin{NiceTabular}{llllllc}
        \CodeBefore
        \rowcolors{1}{}{blue!8}
        \Body
    \toprule
    \toprule
    \textbf{Model Name} & \textbf{Model Arch} & \multicolumn{1}{l}{\textbf{\# of layers }} & \textbf{Training Corpus} & \textbf{Training Objective} & \textbf{URL} & \multicolumn{1}{l}{\textbf{\# of Downloads}} \\
    \midrule
    \textbf{Codegen-2b} & AutoRegressive & 32    & Mono Dataset & Next-token prediction & https://huggingface.co/Salesforce/codegen-2B-mono & 14,558 \\
    \textbf{Codegen-6b-hf} & AutoRegressive & 33    & Mono Dataset & Next-token prediction & https://huggingface.co/Salesforce/codegen-6B-mono & 8,619 \\
    \textbf{Codegen2-1b} & Prefix-LM & 16    & Stack Dataset & Next-token prediction + Fill-in-the-middle prediction & https://huggingface.co/Salesforce/codegen2-1B & 10,783 \\
    \textbf{Codegen2-3.7b} & Prefix-LM & 16    & Stack Dataset & Next-token prediction + Fill-in-the-middle prediction & https://huggingface.co/Salesforce/codegen2-3\_7B & 1,245 \\
    \textbf{Incoder-1b} & XGLMForCausalLM & 24    & GitHub + GitLab + StackOverflow & Causal-masked objective & https://huggingface.co/facebook/incoder-1B & 3,529 \\
    \textbf{Incoder-6b} & XGLMForCausalLM & 32    & GitHub + GitLab + StackOverflow & Causal-masked objective & https://huggingface.co/facebook/incoder-6B & 2,653 \\
    \textbf{Santacoder-1.1} & GPTBigCodeForCausalLM & 24    & Subsets of The Stack  & Next-token prediction + Fill-in-the-middle prediction & https://huggingface.co/TabbyML/SantaCoder-1B & 965 \\
    \textbf{PolyCoder} & GPTNeoXForCausalLM & 32    & GitHub & Next-token prediction & https://huggingface.co/NinedayWang/PolyCoder-2.7B & 731 \\
    \bottomrule
    \bottomrule
    \end{NiceTabular}%
    }
  \label{tab:model}%
\end{table*}%


==> Text/preliminary.tex <==
\section{Preliminary Study}

\input{Preliminary/study}
\input{Preliminary/setup}
\input{Preliminary/results}


